CacheShield: Protecting Legacy Processes Against Cache Attacks

Cache attacks pose a threat to any code whose execution flow or memory accesses depend on sensitive information. Especially in public clouds, where caches are shared across several tenants, cache attacks remain an unsolved problem. Cache attacks rely on evictions by the spy process, which alter the execution behavior of the victim process. We show that hardware performance events of cryptographic routines reveal the presence of cache attacks. Based on this observation, we propose CacheShield, a tool to protect legacy code by monitoring its execution and detecting the presence of cache attacks, thus providing the opportunity to take preventative measures. CacheShield can be run by users and does not require alteration of the OS or hypervisor, while previously proposed software-based countermeasures require cooperation from the hypervisor. Unlike methods that try to detect malicious processes, our approach is lean, as only a fraction of the system needs to be monitored. It also integrates well into today's cloud infrastructure, as concerned users can opt to use CacheShield without support from the cloud service provider. Our results show that CacheShield detects cache attacks fast, with high reliability, and with few false positives, even in the presence of strong noise.

==> implementation.tex <==
\todo{Add motivation, overview and picture from 'Goals and Challenges'}
\todo{Structure: Overview of tool; Change-point detection; application to our tool; implementation of the tool}

As a result of the previous analysis, we decide to monitor the counters for LLC misses and for total cycles. The former gives us information about the use of the LLC of the protected processes while the latter gives information about when it is running or when it has finished. Based on figure (need to put the figure here or before), the \CS\ module needs the PID of the process we desire to protect and the process protected also needs to know the PID of the \CS\ process. The reason is both processes need to communicate with each other (one needs to inform the other when to watch and other needs to inform the one when there is an attack going on), and that the counters can be attached to gather the data from a single process given its PID. 

On Unix systems, the easiest way to use \CS\ is to use the fork operation, and then to use the \textit{exec} system call to run the module and to give it the PID of the parent process. The parent process then can execute the desired operation while being monitored. In case that the parent process stops or waits for something, \CS\ automatically stops after noticing the parent has not been running for a while. This means that when the parent runs again, it needs to send a ``SIGCONT'' signal to the \CS\ tool. In a similar way, if the tool detects an attack, it can send a signal to inform the parent. On Windows Systems the mechanisms for inter-process communications are slightly different, but the tool can be also adapted.

In order to effectively asses the detection task, we made use of change point detection theory (CPD) ~\cite{Basseville:1993:DAC:151741}. This theory can be used to construct the commonly known as quick detection algorithms, which have been successfully applied for quality control, signal-processing, anomaly or intrusion detection tasks among other problems~\cite{}. The assumption in these scenarios is that the parameters describing the monitored system do not change or change very slowly under normal conditions. The parameters can, however, change at unknown time instants (including at startup) into anomalous conditions. This is where CPD algorithms can be used, when the goal is to determine if there has been a significant change in the characteristic parameters of the monitored system in as little time as possible.

The theory of change point detection leads to the development of efficient algorithms presenting certain optimality properties, in the sense that for a given false-alarm rate (FAR) they minimize the average time it takes to detect the change in the descriptive system's features~\cite{}. These CPD algorithms can be easily implemented, do not require too much memory and, as a consequence do not have significant computation overhead. These methods belong to the ``anomaly detection'' class and are \emph{unsupervised} techniques. Hence, they are well-suited to detect new attacks. All these properties made them very attractive for the attack-detection objective. 
In the following, we describe the parameters of the algorithm and how we assess key issues, such as the choice of models or the use of prior information.

We denote the sequence of observations of the $N$ variables we monitor in parallel as $X(t)=(X_{1}(t),...,X_{N}(t))$ , $t \geq 1$. Before a change occurs, the joint probability distribution (pdf) of the random variables $X_{1},...,X_{N}$ also known as \emph{prechange distribution}, can be denoted as $p_0(X_{1},...,X_{N})$. If a change occurs at an unknown time instant $\lambda$, the observations will follow a different distribution $p_1(X_{1},...,X_{N})$, also called \emph{postchange distribution}. That is, when $t < \lambda$ the observations $X(t)$ will have conditional pdf $p_0(X(t)|X(1),...,X(t-1))$, and pdf $p_1(X(t)|X(1),...,X(t-1))$ for $t \geq \lambda$.  

Under the hypothesis that a change has occurred, the stopping time $\tau$ at which the alarm is triggered gives a measurement of the detection time. It is typically defined as the first time the change sensitive statistic watching the system, exceeds a threshold. Naming $E_0$ and $E_\lambda$ the expectations for the sequence of observations prior and after the change at time $\lambda$ , the average detection delay (ADD) is defined as:

\begin{center}
$ADD_\lambda ( \tau ) = E_\lambda ( \tau - \lambda | \tau	\geq \lambda)$
\end{center}
On the other hand, considering that there has not occurred any alarm, the mean time between false alarms will be given by the expression $E_0 \tau $. As a consequence of this definition, the average frequency of false alarms or false alarm rate (FAR) is defined as:
\begin{center}
$FAR(\tau)=\frac{1}{E_0 \tau }$
\end{center}

For a good detection procedure it is expected low FAR and small values of the expected detection delay. The design of CPD algorithms often involves a trade-off between these two parameters. Page's cumulative sum (CUSUM) detection algorithm~\cite{} is one of the most popular CPD algorithms: with a full-knowledge of the pre-change and post-change distributions it provides an optimal scheme minimizing the worst-case detection delay. Page's CUSUM algorithm utilizes the log-likelihood ratio (LLR) to check the hypothesis that a change occurred, LLR is defined as:  

\begin{center}
$s(t)= ln \dfrac{p_1(X(t)|X(1),...,X(t-1))}{p_0(X(t)|X(1),...,X(t-1))}$
\end{center}

The key property of this ratio is that a change in the parameter under study will also cause a change in the sign of the log-likelihood ratio. In other words, s(t) shows a negative drift before change and a positive drift after change. The relevant information for the detection task lies then in the difference between the value of s and a minimum value. The decision rule is based on a comparison with a threshold $h$: 

\begin{center}
$g_k= S_k - m_k \geq h$
\end{center}
where  
\[
S_k =
\sum_{t=1}^{k}s(t)
\]
\begin{center}
$m_k=\min_{1\leq j \leq k} S_j $
\end{center}

This decision rule can be replaced by the following, which obeys the recursion and whose value for the initial observation is $k=0$.
\begin{center}
$g_k = \max \left \lbrace 0,g_{k-1}+\ln \dfrac{p_1(X(k))}{p_0(X(k))}\right\rbrace \geq h$
\end{center}

Then the detection time for the given threshold is 
\begin{center}
$\tau(h) = \min \left \lbrace k \geq 1 : g_k \geq h \right\rbrace $
\end{center}

Although this first approach considers that both distributions are known, this assumption is usually not true, and as a consequence this proposal has to be adapted for each situation. We may know one distribution in advance or none, so it may be necessary to estimate the parameters of the algorithm during the runtime. As long as the estimators for the distributions and the real observation meet certain convergence conditions, we will be able to fix for example the desired detection delay or the FAR.

While facing the cache attack detection, the attack may start from the very beginning or it may start after a few ``normal'' transactions. Both situations are efficiently managed by the proposed CUSUM algorithm. We assume that each new sample can be classified into one of two different groups or clusters, namely ``attack'' and ``non-attack''. The ``non-attack'' cluster represents how we expect the protected process to behave under normal conditions.
Based on the information we can gain from the counters, this assumption is that after a few samples corresponding to the initialization of the protected process, the number of L3 cache misses will be around 0, then $\mu_{na}=0$. On the other hand, when there is an attack, we have observed that the mean number of misses is $\mu_a$. Then each new sample belonging to the ``attack'' cluster will be around $\mu_a$. The value of $\mu_a$ is unknown and depends on the attack so it needs to be computed and recalculated with each new sample.

If we denote as $miss_i$ each new sample that the \CS\ module gets referring to the protected process, we need to decide if it belongs to one cluster or to the other. To do so, we compute the value of the "probability" that $miss_i$ belongs to each one making use of the distance metric, this way we define the distance from $miss_i$ to $\mu_{na}$ as: 

\begin{center}
$d_{na}(i) = miss_i -\mu_{na}=miss_i$ 
\end{center}

Then, the distance with the "attack" cluster will be 

\begin{center}
$d_{a}(i) = | miss_i -\mu_{a} |$ 
\end{center}

As stated before the value of $\mu_a$ is unknown when we start to monitor the process. We select an arbitrary initial value, and whenever a new sample $miss_i$ is obtained, if $miss_i  \geq 0$ we update the value of $\mu_{a}$ as follows:

\begin{center}
$\mu_{a} = (1-\beta) * \mu_{a} + \beta * miss_i $ 
\end{center}

This method is known as exponentially weighted moving average, where the weight of the older datum decreases exponentially. Also note that this way of estimating the mean of the "attack cluster" makes the the election of the initial arbitrary value irrelevant after collecting a few misses samples \todo{what are misses samples?}, considering that this value is reasonable and in the range of the possible values of the average misses per sample. If we choose an initial value too low, we may trigger false positives, if the initialization step takes longer than expected or if the data gathered has some noisy frames in the beginning, so we recommend the election of an initial value higher than 10, in order to maintain the rate of false positives low, while being able to detect the attack in a reasonable time. We will further discuss the noise tolerance of the proposed detection algorithm in the next section. In our experiments we set $ \beta = 0.05$ and the initial value to 12,5.

Now we are in conditions to define the probability of belonging to each cluster:

\begin{center}
$p_{na}(miss_i ) = \dfrac{d_{a}(i)+1}{| d_{na}(i) |+| d_{a}(i) |}$ 
\end{center}

\begin{center}
$p_{a}(miss_i ) = \dfrac{d_{na}(i)+1}{| d_{na}(i) |+| d_{a}(i) |}$ 
\end{center}

Where the value 1 has been added to avoid divisions by 0 in the LLR calculation that has to be performed as part of the detection algorithm. As a result, for every sample $k$, $k \leq 1$ we can express the detection rule as follows:

\begin{center}
$g_k = \max \left \lbrace 0,g_{k-1}+\log \dfrac{p_{a}(miss_k)}{p_{na}(miss_ik)}\right\rbrace \geq h$
\end{center}

Or equivalently,

\begin{center}
$g_k = \max \left \lbrace 0,g_{k-1}+\log \dfrac{d_{na}(k)+1}{d_{a}(k)+1}\right\rbrace \geq h$
\end{center}

As it can be easily derived from the previous equation and according to the properties of the LLR, when the number of misses is 0 or close to 0, the distance between the sample and the "non-attack" cluster $d_{na}(k)$ will be lower than the distance to the attack cluster $d_{a}(k)$, so the value of the metric $g_k$ decreases or keeps 0. On the other hand, readings from the LLC misses counter approaching to the attack cluster will increase the value $g_k$. The properties of this approach let us choose the threshold based on a minimum detection time we want to achieve. Note that when the error in the estimation of the mean $\epsilon$ approaches to zero, $d_{a}(i)=\epsilon$ also tends to zero, then the increase in the value of $g_k$ is also limited

\begin{center}
$\log \dfrac{d_{na}(k)+1}{d_{a}(k)+1} \leq \log ( \mu_{a} +1) $
\end{center}

As a consequence, the minimum expected detection time for the given threshold h is:

\begin{center}
$\tau_{e}(h) \geq  \dfrac{h}{\log ( \mu_{a} +1) }$
\end{center}

or reformulating this equation, the threshold h, for a minimum expected delay $\tau_{e}$

\begin{center}
$h_{\tau} \leq  \tau_{e}*\log ( \mu_{a} +1) $
\end{center}

The unit of the $\tau_{e}(h)$ is "number of samples", to get the value of detection delay in time units just multiply it by the sampling rate. Taking into account that the most effective cache attacks can extract most of the key with just one execution of the victim, we need to select a sampling rate lower than the execution time of the victim and which allows us to collect enough samples. As the execution time of these algorithms is in the order of few milliseconds, a sampling rate of 100 $\mu s$ is enough to provide evidence of the attack. Note that this frequency can be increased, but this would mean extra load for the system. So, for an expected detection delay of 1ms with a sampling rate of 100 $\mu s$ we can define the threshold as $h=\log ( \mu_{a} +1) $. As a result of this selection of $h$, when the $\mu_{a}$ is recalculated, the threshold should be recalculated too. 

\begin{figure}[h]
\centering
\includegraphics[width=0.49\textwidth,trim={45 0 45 0},clip]{example_prime_probe_aes.eps}
\vspace{-6mm}
\caption{Relevant parameters for the detection task, prime+probe attack on AES}
\label{detection_plot}
%\vspace{-3mm}
\end{figure}

The choice of the threshold $h$ would also determine the tolerance to noisy frames, and as a consequence the false positive rate. In practice, the false positive rate cannot be estimated and has to be measured. 

Add a figure for both attack and non attack different rates??????? .

Should I include a formulation of the algorithm as a function??? as a summary of the implementation.
